Multiple-Play Stochastic Bandits with Shareable Finite-Capacity Arms

We generalize the multiple-play multi-armed bandits (MP-MAB) problem with a shareable arm setting, in which several plays can share the same arm. Furthermore, each shareable arm has a finite reward capacity and a ''per-load'' reward distribution, both of which are unknown to the learner. The reward from a shareable arm is load-dependent, which is the "per-load" reward multiplying either the number of plays pulling the arm, or its reward capacity when the number of plays exceeds the capacity limit. When the "per-load" reward follows a Gaussian distribution, we prove a sample complexity lower bound of learning the capacity from load-dependent rewards and also a regret lower bound of this new MP-MAB problem. We devise a capacity estimator whose sample complexity upper bound matches the lower bound in terms of reward means and capacities. We also propose an online learning algorithm to address the problem and prove its regret upper bound. This regret upper bound's first term is the same as regret lower bound's, and its second and third terms also evidently correspond to lower bound's. Extensive experiments validate our algorithm's performance and also its gain in 5G & 4G base station selection.

==> sections/lower_bounds.tex <==
% !TeX root = ../sharing_bandits.tex

\section{Fundamental Limits of \texttt{MP-MAB-SA} }\label{sec:lower_bound}

In this section, we consider the learning limits of the \texttt{MP-MAB-SA} problem.
We first focus on the service capacity learning task
and rigorously prove the task's sample complexity lower bound.
Then, relying on the new sample complexity result, we prove a nontrivial lower bound on the regret of \texttt{MP-MAB-SA}.

% \textbf{illustrate $\mu\to 0$'s difficulties.}

% \begin{corollary}\label{cor:old_m_sample_complexity}
% 	When all arm $k$'s sample sizes $\tau_{k,t}, \iota_{k,t}$ are greater than $\max\{(72M^2/C^2)\log T, 1/4C^4\}$, we have
% 	\begin{equation*}
% 		\mathbb{P}(\forall k\in [K], {\hat{m}_k} = m_k) \ge 1 - \frac{2K}{T}.
% 	\end{equation*}
% \end{corollary}

% \begin{corollary}\label{cor:m_sample_complexity}
% 	When all arm $k$'s sample sizes $\tau_{k,t}, \iota_{k,t}$ are greater than $\max\{(72M^2/C^2)\log (2K/\delta), 1/4C^4\}$, we have
% 	\begin{equation*}
% 		\mathbb{P}(\forall k\in [K], {\hat{m}_k} = m_k) \ge 1 - \delta.
% 	\end{equation*}
% 	% Question: can we write the sample complexity as $O(M^2 (1/C^2)\log(1/\delta))$ as there is a max between $1/4C^2$?
% \end{corollary}
\subsection{Sample Complexity Lower Bound}

The challenges of learning service capacity \(m_k\) lie in the load-dependent reward feedback (Eq.(\ref{eq:arm_level_feedback})) and heterogeneous explorations.
As the feedback depends on the random variable \(X_k\) multiplying the uncertain factor \(\min\{a_{k,t}, m_k\}\), one cannot easily discern whether the number of plays \(a_{k,t}\) is greater than the capacity \(m_k\) or not, let alone the service capacity \(m_k\).
Furthermore, the shareable arm setting allows any number of plays to pull an arm.
That is, for each arm there can be many types of explorations, which further complicates the learning task.

% We show that with some simplifications and restrictions, the service capacity learning task can be reduced to a simpler task.
% From that, we prove the task's sample complexity lower bound in Theorem~\ref{thm:sample_lower_bound}.
Although the learning task is challenging, we show that, with some prior knowledge and an restriction, it can be reduced to
a much simpler task.
This simplification helps us to derive the task's sample complexity lower bound.
%  in Theorem~\ref{thm:sample_lower_bound}.

% \textbf{To smooth the illustration of the rest of this paper, we define united exploration (UE) and
%     individual exploration (IE) here. }

% {Our estimation is built on two kinds of explorations: when an arm is played by a number of plays \(a_{k,t}\) below its capacity \(m_k\), and when the number of plays exceeds its capacity.
%     Note that one cannot distinguish both cases from the reward observations.
%     One coarse approach is using extreme number of plays to explore, i.e., assign \(1(<m_k)\) play or \(N(\ge m_k)\)
%     plays. Later, our algorithm (at Section~\ref{sec:opt_algorithm}) employs the capacity's confidence bounds to better differentiate them.}

% When $a_{k,t}< m_k$, the observed reward divided by $a_{k,t}$
% is a sample of ``per-load'' reward  $X_k$ and
% can be used to estimate its mean $\mu_k$.
% When $a_{k,t}\ge m_k$, the reward is a sample of ``full-load'' reward $m_k X_k$ and
% can estimate its mean $m_k\mu_k$.
% % The former can be used to estimate the reward mean $\mu_k$ and the later for $m_k\mu_k$. 
% We name the former as \textbf{individual exploration (IE)} and the latter as \textbf{united exploration (UE)}\footnote{Note that we abuse UE of Section~\ref{sec:lower_bound} to represent all explorations with \(a_{k,t}\ge m_k\) as their observations are equivalent.}.
% We define $\tau_{k,t}$ to record the number of IEs up to time slot $t$,
% $S_{k,t}^{\text{IE}}$ as the associated total ``per-load'' reward samples,
% and $\hat{\mu}_{k,t}$ as the ``per-load'' reward's sample mean:
% \(\tau_{k,t} \coloneqq   \sum_{s=1}^t
% \mathds{1}\{a_{k,s} < m_k\},
% S_{k,t}^{\text{IE}} \coloneqq \sum_{s=1}^t ({R_{k,s}}/{a_{k,t}})\mathds{1}\{a_{k,s} < m_k\}\),
% and \(\hat{\mu}_{k,t} \coloneqq {S_{k,t}^{\text{IE}}}/{\tau_{k,t}}\).

% Similarly, we define $ \iota_{k,t}$, $S_{k,t}^{\text{UE}} $, and ``full-load'' reward's sample mean $\hat{\nu}_{k,t}$ for UEs: \(\iota_{k,t} \coloneqq
% \sum_{s=1}^t  \mathds{1}\{a_{k,s} {\ge} m_k\}, S_{k,t}^{\text{UE}} \coloneqq  \sum_{s=1}^t  R_{k,s} \mathds{1}\{a_{k,s} {\ge} m_k\},\) and \(\hat{\nu}_{k,t} \coloneqq  {S_{k,t}^{\text{UE}}}/{\iota_{k,t}}.\)

\begin{theorem}[Sample Complexity Lower Bound]\label{thm:sample_lower_bound}
    Denote \(\sigma_k^2\) as the variance of arm \(k\)'s ``per-load'' reward \(X_k\) and that \(\sigma_k^2 \ge 50\mu_k^2/m_k\).
    If the exploration times\footnote{Note that one exploration can have any number of plays pulling the same arm.} of arm \(k\) is less than \[({12\sigma_k^2 m_k^2}/{\mu_k^2})\log\left( {c}/{\delta} \right),\] where \(c\) is a universal constant,
    then there exists some ``per-load'' reward distributions over \(X_k\) such that
    the probability of falsely estimate the capacity is no less than \(\delta\), or formally, \(\P(\hat{m}_{k} \neq m_k)\ge \delta\).
\end{theorem}
\vspace{-1\baselineskip}
\begin{proof}[Proof Sketch of Theorem~\ref{thm:sample_lower_bound}]
    The detailed proof is in Appendix~\ref{app:sample_lower_bound}.
    \textit{Step~(1): assuming on prior knowledge.}
    Assume the ``per-load'' reward \(X_k\)'s mean \(\mu_k\) is known a priori.
    With the additional knowledge, the simplified task's lower bound is no greater than the original task's.
    \vspace{-0.25\baselineskip}

    \noindent\textit{Step~(2): exploration restriction.}
    Explorations are restricted to united explorations
    --- simultaneously assigning all \(N (\ge m_k)\) plays to explore arms.
    United explorations can generate samples from ``full-load'' reward \(m_kX_k\).
    We note that this restriction does not vary the difficulty of the learning task:
    The samples from explorations with plays less than the capacity, i.e.,  \(a_{k,t}<m_k\),
    are \textit{not as effective as} samples from united exploration.
    %  learning \(m_k\),
    Because without known \(m_k\) one still needs to discern whether \(a_k<m_k\) or not
    even the mean \(a_{k,t}\mu_k\) is assumed to be known in \textit{Step~(1)}.
    For other explorations that \(a_{k,t}\ge m_k\), their observations are sampled from \(m_kX_k\) and thus are equivalent to united explorations. \vspace{-0.25\baselineskip}

    \textit{Step~(3): the reduced task.}
    After above two steps, this learning task is reduced to estimate the empirical mean \(\hat{\nu}_k\) of united explorations' reward \(m_k X_k\).
    Because the mean \(\hat{\nu}_k\) is an estimate of \(m_k\mu_k\) and, after divided by the known \(\mu_k\), is an estimate of the service capacity \(m_k\). \vspace{-0.25\baselineskip}

    \textit{Step~(4): anti-concentration.}
    Since the capacity \(m_k\) is an integer, the event \(\abs{(\hat{\nu}_k/\mu_k) - m_k}\ge 1/2\)  is equivalent to \(\hat{m}_{k}\neq m_k\).
    With an anti-concentration inequality (cf.~\cite{matouvsek2001probabilistic}), we prove that the probability of the former event is no less than \(c\exp(-{\mu^2_k n}/{12m_k^2\sigma_k^2})\), where \(n\) is the number of times of united explorations.
    Making the exponential expression greater than \(\delta\) leads to the sample complexity lower bound.
\end{proof}

Theorem~\ref{thm:sample_lower_bound} states that to correctly estimate an arm's service capacity with \(1-\delta\) confidence, one needs at least \(\Omega((m_k^2/\mu_k^2)\log(1/\delta))\) times of explorations.
In Section~\ref{sec:learning_sharing_capacity}, we will devise an estimator whose sample complexity upper bound can match the lower bound up to a constant factor.
This important result shows that the lower bound derived in Theorem~\ref{thm:sample_lower_bound} is nearly optimal.

\subsection{Regret Lower Bound}
Next, we provide an asymptotical regret lower bound for the \texttt{MP-MAB-SA} problem in Theorem~\ref{thm:regret_lower_bound}.
Part of the proof is based on Theorem~\ref{thm:sample_lower_bound} (see Appendix~\ref{app:regret_lower_bound} for detail).

\begin{theorem}[Regret Lower Bound]~\label{thm:regret_lower_bound}
    For any consistent\footnote{Please refer to Definition~\ref{def:consistent} in Appendix~\ref{app:regret_lower_bound}.} algorithm to address the \texttt{MP-MAB-SA} problem with \(K\) arms and \(L\) optimal arms and in its optimal action the least favored optimal arm \(L\) is shared by more than one plays,
    its regret is lower bounded as:
    % For any \emph{\texttt{MP-MAB-SA}} problem with $K$ arms and optimal actions containing $L$ arms, the regret to address it is lower bounded as:
    \begin{equation*}
        \liminf_{T\to \infty}\frac{\ERT}{\log T} \ge \sum_{k=L+1}^K \frac{\Delta_{L,k}}{\KL(v_k, v_L)} +
        C\sum_{k=1}^L\frac{\sigma_k^2 m_k^2}{\mu_k^2}.
    \end{equation*}
    where \(C\le 12\min_{1\le k\le K-1} \Delta_{k,k+1}\) is a positive constant, $\KL(\cdot,\cdot)$ is KL-divergence and $v_k$ is the ``per-load'' reward \(X_k\)'s distribution.
\end{theorem}

% \begin{proof}[Proof Sketch of Theorem~\ref{thm:regret_lower_bound}]
%     The detailed proof is in Appendix~\ref{app:regret_lower_bound}.
%     \textit{Step (1): regret lower bound of exploring suboptimal arms.} To Do

%     \textit{Step (2): regret lower bound of learning optimal arms' service capacities.} To Do
% \end{proof}

The regret lower bound of Theorem~\ref{thm:regret_lower_bound} contains two terms.
The first term corresponds to the classic regret of bandits problem~\citep{anantharam1987asymptotically}.
Specifically, we note that for Bernoulli ``per-load'' reward \(X_k\),
the first term is of the order \(\Omega(\sum_{k=L+1}^K (1/\Delta_{L,k}))\).
The second term is due to the cost of learning optimal arms' service capacities
which is quantified by Theorem~\ref{thm:sample_lower_bound}'s sample complexity lower bound.

==> sections/the_se_algorithm.tex <==
% !TeX root = ../sharing_bandits.tex
\section{The \texttt{MP-SE-SA} Algorithm}\label{sec:algorithm}

%In this section, we present our \texttt{MP-SE-SA} algorithm for the multi-play MAB with sharable arms.
We first present the high level idea of our \texttt{MP-SE-SA} algorithm.
Then, we explain the successive elimination (SE) framework
and provide detailed description of \texttt{MP-SE-SA}.

\subsection{Design Overview}
% One cannot easily adapt index policies like upper confidence bound (UCB)~\citep{auer2002finite}, or Thompson sampling (TS)~\citep{thompson1933likelihood} to solve \texttt{MP-MAB-SA}.
% These index policies are deliberately designed for estimating reward means (or other statistics) from
% reward random variables'  realizations.
% But there is no such random variable supplying realizations for the service capacity.
% % , which invalids these index policies.
% Furthermore, even if one can obtain capacities' confidence bounds or other statistics (we do propose such a technique in this paper), under the exploration and exploitation dilemma,
% applying index policies to tackle the coupling between learning capacity and reward mean is still challenging.
% The reason is that index policies (e.g., UCB) can only handle the dilemma caused by reward alone.
% In other words, one may not be able to have good results using the classical index policies.

% In a word, designing an index policy that can handle these two coupled tasks as a whole is highly perplexing (if not impossible).

% Designing an efficient algorithm for \texttt{MP-MAB-SA} requires one not only
% to partially separate both coupled learning tasks,
% %  so as to make the problem solvable, 
% but also to maintain a connection between both tasks in order to have a fine-grained learning efficiency.
% As index policies are inapplicable and coarse-grained approaches (like explore-then-commit (ETC)) can be costly~\citep{garivier_explore-then-commit_2016},
% one has to seek an approach which can decouple
% % that is both capable of decoupling 
% both tasks and is flexible enough for fine-grained level operations.
% The successive elimination (SE) framework fulfills such requirements.
% SE was first introduced to MAB by~\citet{even2006action} in best arm identification problem and then further analyzed by~\citet{perchet_multi-armed_2013}, which guarantees its good performance.
% % we develop our algorithms based on successive elimination (SE).
% Also, it only relies on an elimination condition and thus allows a far more flexible design than ETC. With SE's capability and flexibility, we propose the multiple-play successive elimination with shareable arms (\texttt{MP-SE-SA}) algorithm, which uses a uniform confidence interval (UCI) for capacity estimate to gradually reduce the expected number of top arms one should reserve, and successively eliminate suboptimal arms.



Besides the exploration vs. exploitation trade-off,
the main challenge of the \texttt{MP-MAB-SA} problem is its
% As we show in introduction, our \texttt{MP-MAB-SA} problem's challenge comes from its 
two coupled learning tasks:
(1) learning each arm's per load reward mean, (2) learning each arm's service capacity.
% In addition, one also needs
% % Besides their coupling, we also need 
% to deal with the exploration and exploitation trade-off.
%  as the MAB problem.

One typical approach is to deal with \textit{these coupled learning tasks as a whole}, e.g., assign plays according to the UCB indexes of the capacities and reward means.
However, we note that opportunistic estimating the capacity $m_k$ (via UCB) cannot easily balance exploitation and exploration because $\hat{m}_{k,t}$ is \emph{not} estimated as the mean of a distribution while the reward mean $\hat{\mu}_k$ does.
% That invalids these index policies.
% and the wrong capacity also invalidates the UCB of per play reward means.
% because over or under estimating capacity
% leads to sub-optimal assignment of plays.
An alternative is to
\textit{separate the two coupled learning tasks
    as independent ones},
for example,
one first individually and unitedly explores
% $K(1/N{+}\ceil{{K}/{N}}){\times}\O(N^2\log T)$ time slots\footnote{
% 	$\O(N^2\log T)$ is the sample complexity from Corollary~\ref{cor:m_sample_complexity}, where we set $m_k$ to $N$ as its upper bound, and omit $\mu_k$.
% }
all $K$ arms to estimate their capacities,
% accurately,\footnote{That is, use IE to estimate $\hat{\mu}_{k,t}$ and UE for $\hat{\nu}_{k,t}$, and then apply estimator $\hat{m}_{k,t}$ in Eq.(\ref{eq:rounding_estimator}).}
and then adapts UCB
to the \texttt{MP-MAB-SA} with known capacity setting to update per load reward mean estimates.
We name this two-phase strategy as \texttt{ETC-UCB}.
This is a simple, yet inefficient, algorithm.
Because when the number of arms $K$ is much greater than the number of plays $N$,
% i.e., $K\gg N$, 
there would be a great cost 
in learning the $K-N$ suboptimal arm's service capacities which turns out to be unnecessary.
We present the algorithm's detail and regret upper bound analysis in Appendix~\ref{app:etc_ucb}.

% causes a $\O((K^2N{+}KNM)\log T)$
% regret (see Appendix~\ref{appsub:etc_ucb}).
% \footnote{Draft:
%     % the latter part should be updated, CUCB is much complex than $1/\Delta^2$.
%     the proof is done. But still need to check.
% } 
% However, this exploration strategy is crude and not efficient.
%In Section~\ref{sec:analysis}, we show that our algorithm enjoys much smaller coefficients.
%
%The above two approaches either regard these two coupled tasks as a whole 
%(i.e., the UCB method)   
%or clearly separate them as two independent parts (i.e., ETC method).  
%As UCB is inapplicable and ETC is crude and inefficient,

A better approach should \emph{partially} separate (decouple) \texttt{MP-MAB-SA}'s two learning tasks,
% so as to be feasible, and 
but also utilize their relations to improve the efficiency,
% to partially separate both coupled learning tasks,
% %  so as to make the problem solvable, 
% but also utilize their relations to improve the efficiency.
% As index policies are inapplicable and coarse-grained approaches (like explore-then-commit (ETC)) can be costly~\citep{garivier_explore-then-commit_2016},
which needs an approach
% which can decouple
% % that is both capable of decoupling 
% both tasks but 
that is flexible enough for fine-grained level operations.
% The successive elimination (SE) framework fulfills such requirements.
We extend successive elimination (SE)~\citep{perchet_multi-armed_2013} to achieve that.
Our algorithm design has two challenges.
First, applying SE to handle the exploration vs. exploitation trade-off with multiple plays
is more complicated than single play MAB.
In particular, it also needs to balance two types of explorations: individual exploration (IE) and united exploration (UE).
Second,
% instead of knowing the required number of top arms in MP-MAB,
% our MAB setting with sharable arms and multiple plays,
the number of arms $L$ that should be reserved from elimination is unknown in advance.
% IF eliminating too much arms, left arms will be insufficient, leading to a linear regret.
% IF eliminate too less arms, we have to explore suboptimal arms often which also leads to additional costs.
Specifically, it can only be determined by the reward means' rank and their capacities, both of which are unknown a priori.
% Also, multiple plays in each round make the exploration more complicated.
% One needs to decide the number of plays for each arm,
% which influences the estimation of shareable capacity and per play reward mean.
% Later, we propose \emph{two criteria} to tackle them respectively.

% We illustrate our \texttt{MP-SE-SA} algorithm as follows. We first provide the successive elimination framework adapted from~\citep{perchet_multi-armed_2013} and provides a coarse-grained method to determine how many arms we should eliminate.
% Then, we show a fine-grained update strategy which meets the desirable approach's requirements: partially separate both tasks but still utilize their correlation.
% Finally, we show the \texttt{MP-SE-SA} algorithm.

\subsection{The Successive Elimination Framework}

Recall that
%whose capacities together can cover all $N$ plays,
% with an assumed descending per play reward mean order,
the optimal arm set is $[L]\coloneqq\{1,2,\ldots, L\}$
and the rest arms are {suboptimal},
where $L$ is defined in Eq.(\ref{eq:critical_top_arms})
as the number of arms pulled in the optimal action.
The main idea of our algorithm is as follows.
We initialize a candidate set $\mathcal{S}_t = [K]$.
In each exploration round,
we uniformly explore
% (IE or UE determined by the algorithm) 
each arm in $\mathcal{S}_t$
and then use their rewards to update estimates of reward means and capacities.
In the process, we eliminate suboptimal arms from $\mathcal{S}_t$
according to \textit{two criteria} (see below) until $\mathcal{S}_t=[L]$.
As all arms $k\in\mathcal{S}_t$ have the same rounds of IE $\tau_{k,t}$ and UE $\iota_{k,t}$,
we omit their subscript $k$ as $\tau_t$ and $\iota_t$.
Denote reward mean estimate $\hat{\mu}_{k,t}$'s descending order map as $\sigma_t(\cdot)$.

\textbf{The elimination criterion.}
The first criterion is to accurately eliminate suboptimal arms with an opportune number of explorations (i.e., avoid over explorations).
This relies on reward mean estimates $\hat{\mu}_{k,t}$ and
the following elimination condition.
% We extend the elimination condition proposed for MAB by~\citet{perchet_multi-armed_2013} to multiple-play setting. 
For any arm $k$ in the candidate set $\mathcal{S}_t$, if its reward mean estimate $\hat{\mu}_{k,t}$ is much worse than the ${L}^{\text{th}}$ largest\footnote{The $L$ is estimated in the second criterion's Eq.(\ref{eq:update_L_with_lower_bound}).}, i.e.,
%  fulfill the following inequality
\begin{equation*}
    \hat{\mu}_{k,t} \le \hat{\mu}_{\sigma_t(L),t} - U(\tau_t, T),
\end{equation*}
we eliminate the arm $k$ from $\mathcal{S}_t$. The function $U(\tau_t, T)$ is a high confidence upper bound on the deviation of $\hat{\mu}_{k,t} - \hat{\mu}_{\sigma_t(L),t}$ from $\mu_k - \mu_{\sigma_t(L)}$, and it is expressed as
%  and $\tau_t$ is the IE times for the candidate set.
% The $U(\tau_t, T)$ is
% \begin{equation}
% \label{equ:mu_interval_width}
$
    U(\tau_t, T) \coloneqq 2\sqrt{ 2 \tau^{-1}_t \xoverline{\log} \left(T/\tau_t \right)},
$
where $\xoverline{\log}(x) = \max\{\log x, 1\}$.
% for any two arm $k  > l$ both with $\tau$ times of IE, that's a high confidence upper bound on the deviation of $\hat{\mu}_{k,t} - \hat{\mu}_l$ from $\mu_k - \mu_l$.
%  and $a\vee b = \max\{a,b\}$.	
% make sure the confidence interval width is less than half to guarantee the correct estimation. 

% only containing the top-$L$ arms (i.e. $\mathcal{S}_t$ equal to $[L]$).
% maintain a candidate arm set $\mathcal{S}_t$ initialized as the whole arm set $[K]$, and  
% The algorithm's aim is to reduce candidate arm set's size $\abs{\mathcal{S}_t}$ to $L$ both effectively and safely (i.e., with high correct probability). 


\textbf{The over elimination avoidance criterion.}
The second criterion is to assure that the total capacity of remaining arms in the candidate set $\mathcal{S}_t$
% 's all arms' capacities
%  (in set $\mathcal{S}_t$) 's arms' 
% the shareable capacities $m_k$
% of arms in the candidate set $\mathcal{S}_t$ 
can cover $N$ plays, i.e., avoid any over elimination.
This depends on capacity estimates $\hat{m}_{k,t}$ and their uniform confidence interval (UCI).
% $W(\tau_{t}, \iota_{t}, 1/T)$, where the confidence $\delta$ is set as $1/T$.
Denote $\hat{L}_t$ as the expected size of $\mathcal{S}_t$ at time $t$.
It assures that with observations up to time $t$, the total capacities of top $\hat{L}_t$ arms in $\mathcal{S}_t$ is no less than $N$. So, we can achieve this criterion as long as the
size $\abs{\mathcal{S}_t}$ is no less than $\hat{L}_t$.

% One approach for setting the size $\hat{L}_t$ is as follows. When we cannot estimate the capacity accurately, we set $\hat{L}_t=N$ so to enable $\mathcal{S}_t$ to cover $N$ plays.
% % to make sure that $\mathcal{S}_t$ can always bear at least $N$ plays without exceeding any arm's limit.
% When capacity estimate $\hat{m}_{k,t}$ reaches the confidence $1/T$,
% we obtain the final size
% \begin{equation}\label{eq:update_L_at_last}
% 	\hat{L}_t
% 	=
% 	\argmin_n\left\{n: \sum_{k=1}^n \hat{m}_{\sigma(k),t} \ge N\right\},
% \end{equation}
% and with high probability, $\hat{L}_t= L$.
% This update is like a step function as $\hat{L}_t$ abruptly reduces from $N$ to $L$
% when $\hat{m}_{k,t}$ reaches the confidence level.
% % , which is coarse.
% We name this approach as the \emph{``coarse-grained update''} method.

% 	%\subsection
% {\bf A fine-grained update for expected candidate set size.}
A key element of our algorithm design is to efficiently reduce the expected size $\hat{L}_t$.
% As mentioned beFore, we should make sure the top $\hat{L}$ arms' shareable capacities can cover all $N$ plays.
% With the same initial and final $\hat{L}_t$ as the coarse-grained update,
% the \emph{fine-grained update} utilizes the capacity estimator's UCI.
At the beginning, we set $\hat{L}_t=N$ since $N$ arms cover at least $N$ plays.
As the algorithm proceeds, we update capacities' lower and upper bounds:
\begin{equation}\label{eq:m_lower_bound}
    \hat{m}_{k,t}^{l}=\max\!\left\{\!\ceil{\!\frac{\hat{\nu}_{k,t}}{\hat{\mu}_{k,t} + \phi(\tau_{t},\delta) + \phi(\iota_{t},\delta)}\!}\!, \hat{m}_{k,t-1}^{l}\!\right\}\!,
\end{equation}
\begin{equation}\label{eq:m_upper_bound}
    \hat{m}_{k,t}^{u}=\min\!\left\{\!\floor{\!\frac{\hat{\nu}_{k,t}}{\hat{\mu}_{k,t} - \phi(\tau_{t},\delta) - \phi(\iota_{t},\delta)}\!}\!, \hat{m}_{k,t-1}^{u}\!\right\}\!,
\end{equation}
for all arm $k$ in $\mathcal{S}_t$. We then use $\hat{m}_{k,t}^{l}$ to update $\hat{L}_t$,
% Denote empirical per play reward means' order descending map as $\sigma_t(\cdot)$.
\begin{equation}\label{eq:update_L_with_lower_bound}
    \hat{L}_t
    =
    \min\left\{n: \sum\nolimits_{k=1}^n \hat{m}_{\sigma(k),t}^{{l}} \ge N\right\}.
\end{equation}
% Later on, when $W(\tau_t, \iota_t, 1/T) < 1/2$, the estimations of shareable capacities as $\hat{m}_{k,t}$
% becomes accurate enough. We then obtain the smallest expected size
% \begin{equation}\label{eq:update_L_at_last}
% 	\hat{L}_t= \argmin_n\left\{n, \sum_{k=1}^n \hat{m}_{\sigma(k),t} \ge N\right\},
% \end{equation}
% and with high probability, $\hat{L}_t= L$.
Figure~\ref{fig:size_update} depicts the expected size $\hat{L}_t$'s update and compares it with \texttt{ETC-UCB} (in Appendix~\ref{appsub:etc_ucb_alg}).
The improvements of the \texttt{MP-SE-SA} algorithm are two folds:
(1) it only performs united explorations on top $N$ arms after eliminating $K-N$ obviously inferior arms (see the blue shadow), 
(2) it gradually reduces the expected arm size $\hat{L}_t$ in exploration rounds, which further avoids learning exact capacities for the rest $N-L$ suboptimal arms (see the orange shadow).
% With the uniformly applicable UCI, we can reduce the expected size within all exploration rounds.
% The improvement of the coarse-grained update over the ETC is from the elimination:
% we eliminate obviously suboptimal arms, and perform explorations on potentially good ones.
%  the cost of exploration.
% We omit the variable $t$ of $\hat{L}_t$ when no confusion is possible.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/L_comparison.pdf}
    \caption{The update of candidate set's expected size $\hat{L}_t$}
    \label{fig:size_update}
\end{figure}
% \vspace{-1cm}

\subsection{The \texttt{\texttt{MP-SE-SA}} Algorithm}
\setlength{\textfloatsep}{0pt}
\begin{algorithm}[htb]
    \caption{Multiple-play successive elimination with shareable arms (\texttt{MP-SE-SA})}
    \label{alg:main}
    {\bfseries Input:} $K$, $N$, $T$ and parameters $\gamma \in [1, \infty), \xi \in (0, \infty).$\\
    {\bfseries Initial:}
    \(t,\tau_t,\iota_t, \gets 1, \mathcal{S}_t \gets [K],\delta\gets 2\xi/T, \hat{\bm{\mu}}_t,\hat{\bm{\nu}}_t \gets\bm{0}, \hat{\bm{m}}_t^l \gets \{1,\ldots,1\}, \hat{\bm{m}}_t^u \gets \{N,\ldots,N\},
    \hat{L}_t\gets N.\)
    \begin{algorithmic}[1]
        % \STATE {\bfseries Input:} Arm set $[K]$, Multiple-Play $N$, time horizon $T$, and parameters $\gamma\in (1,\infty)$ and $\xi\in (0,1).$   	
        \WHILE{$t\le T$}
        % \STATE \multiline{Update the descending ordering $\sigma_t(\cdot)$ such that $\hat{\mu}_{\sigma_t(k),t}$ is the $k$th largest in $\{\hat{\mu}_{k,t}, k \in \mathcal{S}_t\}$.}
        \STATE {Update the descending ordering $\sigma_t(\cdot)$ such that $\hat{\mu}_{\sigma_t(k),t}$ is the $k$th largest in $\{\hat{\mu}_{k,t}, k \in \mathcal{S}_t\}$.}
        \STATE{Update the expected set size $\hat{L}_t$ by Eq.(\ref{eq:update_L_with_lower_bound}). \label{alg:line:update_L}}
        \IF{$\hat{L}_t< \abs{\mathcal{S}_t}$}\label{alg:line:L<S}
        \STATE{\textsc{Elimination}($\mathcal{S}_t, \hat{\bm{\mu}}_t, \hat{L}_t, \sigma_t(\cdot),\gamma,T$).}\label{alg:line:eliminate}

        \STATE{\scshape Individual Exploration($\mathcal{S}_t, \hat{\bm{\mu}}_t, \tau_t, t$).}\label{alg:line:ie}
        \ELSIF{$\hat{L}_t= \abs{\mathcal{S}_t}$}\label{alg:line:L=S}
        \STATE{\scshape Exploitation($\mathcal{S}_t,\hat{\bm{m}}_t^l,\hat{\bm{\mu}}_t,\hat{L}_t,\sigma_t(\cdot),\tau_t, t$).}\label{alg:line:explore}

        \STATE{$\mathcal{S}_t'\gets\{k\in\mathcal{S}_t:\hat{m}_{k,t}^l\neq\hat{m}_{k,t}^u\}.$}\label{alg:line:S_prime}
            \IF{\(\mathcal{S}_t' \neq \emptyset\)}
            \STATE{\scshape United Exploration($\mathcal{S}_t', \hat{\bm{\nu}}_t, \iota_t, t$).}
            \label{alg:line:ue}
            \STATE{Update $\hat{{m}}_{k,t}^l$ and $\hat{{m}}_{k,t}^u$ by Eq.(\ref{eq:m_lower_bound})(\ref{eq:m_upper_bound}).} \label{alg:line:update_m}
            \ENDIF
        \ENDIF
        \ENDWHILE
        \end{algorithmic}
    \end{algorithm}
    % \vspace{-3cm}

We present \texttt{MP-SE-SA} in Algorithm~\ref{alg:main}.
% The expected candidate arm set size $\hat{L}_t$ is the indicator of \texttt{\texttt{MP-SE-SA}} algorithm.
The magnitude of the current candidate arm set size $\abs{\mathcal{S}_t}$ comparing to the expected size $\hat{L}_t$ directs the \texttt{\texttt{MP-SE-SA}} algorithm.
That $\hat{L}_t<\abs{\mathcal{S}_t}$ (Line~\ref{alg:line:L<S})
implies the candidate arm set $\mathcal{S}_t$ containing suboptimal arms.
Then, the algorithm repeatedly employs IEs to the arms in $\mathcal{S}_t$ (Line~\ref{alg:line:ie}) so as to distinguish suboptimal ones and eliminate them (Line~\ref{alg:line:eliminate}).
After eliminating the $\abs{\mathcal{S}_t}-\hat{L}_t$ suboptimal arms, $\hat{L}_t = \abs{\mathcal{S}_t}$ (Line~\ref{alg:line:L=S}) and the algorithm turns to exploit the current arm set (Line~\ref{alg:line:explore}).
In the scenario, for arms whose capacity have not been exactly learnt, i.e., in set $\mathcal{S}_{t}'$ at Line~\ref{alg:line:S_prime}, the algorithm employs UEs to acquire samples for estimating the full load mean $m_k\mu_k$ (Line~\ref{alg:line:ue}) and update the $\hat{{m}}_{k,t}^l$ and $\hat{{m}}_{k,t}^u$ estimates (Line~\ref{alg:line:update_m}).
Then $\hat{L}_t$ may decrease accordingly (Line~\ref{alg:line:update_L}) and the algorithm may go back to the $\hat{L}_t<\abs{\mathcal{S}_t}$ case.
Finally, when $\hat{L}_t=\abs{\mathcal{S}_t}$ and the capacities of arms in $\mathcal{S}_t$ are learnt ($\mathcal{S}_t'{=}\emptyset$),
the algorithm finds the optimal arm set, i.e., $\mathcal{S}_t{=}[L]$ and, from then on, settles down on the optimal action.

% In Line~\ref{alg:line:S_prime}, We construct a set $\mathcal{S}_t'$ as a subset of $\mathcal{S}_t$ consisting of arms whose capacities' estimation criterion hasn't been fulfilled. Because once an arm's estimation criterion is achieved, we obtain its capability with high probability. 
% Line~\ref{alg:line:ue} adds another condition $\abs{\mathcal{S}_t}\le N$. It means that the algorithm only starts to do united exploration after the worst $K-N$ arms are eliminated. For one thing, the expected candidate arm set size $\hat{L}_t$ is initialized $N$. 
% When $\abs{\mathcal{S}_t} > N$,  
% there is no need to acquire UE observations for reducing $\hat{L}_t$. 

To enhance the algorithm's efficiency, we add two parameters: $\gamma \ge  1$ for scaling elimination's deviation gap as $\gamma U(\tau_t, T)$ and $\xi > 0$ for tuning UCI's confidence level $1-\delta$ as $1 - 2\xi/T$.
The smaller the $\gamma$, the more aggressive in eliminating arms, while the smaller the $\xi$, the more conservative in estimating capacities.
$\gamma$ and $\xi$ can be tuned for better performance in a specific environment but simply setting both as $1$ is also valid.
Their impact on regret is shown analytically in Theorem~\ref{thm:main_regret} and empirically in Appendix~\ref{appsub:impact_of_gma_xi}.
% Other subroutines of Algorithm~\ref{alg:main} including individual exploration in PROCEDURE~\ref{alg:ie}, united exploration in PROCEDURE~\ref{alg:ue}, and exploitation in PROCEDURE~\ref{alg:exploitation} are deferred to Appendix~\ref{appsub:procedures}.
% \footnote{Draft: or we can move these last three procedures to Appendix, as they are too trivial to occupy space.}.
% Apart from the SE framework and fine-grained update above, 


{\texttt{MP-SE-SA}'s four procedures are presented in Algorithm~\ref{alg:procedures}.
The \textsc{Elimination} procedure at Line~\ref{proc:elimination} corresponds to \textbf{the elimination criterion} in the previous subsection. 
The \textsc{Individual Exploration} procedure (Line~\ref{proc:ie}) collects samples for estimating candidate arms' per load reward mean \(\mu_k\). 
It evenly divides the current candidate arm set \(\mathcal{S}_t\) to \(\ceil{\abs{\mathcal{S}_t}/N}\) subsets so that each of them contains no more than \(N\) arms (Line~\ref{proc:ie:divide}). 
In each time slot, the procedure assigns plays to individually explore arms of one subset (Line~\ref{proc:ie:ie}).
% , observe rewards, and update their pre load reward mean estimates \(\hat{\mu}_{k,t}\).
The \textsc{United Exploration} procedure (Line~\ref{proc:ue}) collects samples for estimating the full load reward mean \(m_k\mu_k\) of candidate arms whose capacities have not been learnt, i.e., in \(\mathcal{S}_t'\). 
It assigns all \(N\) plays to pull each arm in \(\mathcal{S}_t'\) in turn (Line~\ref{proc:ue:ue}).
% , observe rewards, and update their full load reward mean estimates \(\hat{\nu}_{k,t}\).
The \textsc{Exploitation} procedure (Line~\ref{proc:exploitation}) assigns plays to maximize expected reward according to the estimated per load reward \(\hat{\mu}_{k,t}\) and capacities' lower confidence bounds \(\hat{m}_{k,t}^l\).}
% , observe rewards, and updates the estimates \(\hat{\mu}_{k,t}\). 
    \begin{algorithm}[htb]
            \caption{Procedures of \texttt{MP-SE-SA}}
            \label{alg:procedures}
            \begin{algorithmic}[1]
        \PROCEDURE{Elimination}{$\mathcal{S}_t, \hat{\bm{\mu}}_t, \hat{L}_t, \sigma_t(\cdot),\gamma,T$} \label{proc:elimination}
        \FORALL{$k\in \mathcal{S}_t$ }
        \IF {$\hat{\mu}_{k,t} \le \hat{\mu}_{\sigma(\hat{L}_t),t} - \gamma U(\tau_t, T)$}
        \STATE $\mathcal{S}_t\gets \mathcal{S}_t\setminus\{k\}.$ \label{line:elimination}
        \ENDIF
        \ENDFOR
        \ENDPROCEDURE

        \PROCEDURE{Individual Exploration}{$\mathcal{S}_t,\!\hat{\bm{\mu}}_t,\! \tau_t,\! t$} \label{proc:ie}
        % \STATE {\bfseries Input:} Candidate arm set $\mathcal{S}_t$, empirical mean $\hat{\bm{\mu}}$  
        % \STATE{Divide $\mathcal{S}_t$ to $\ceil{\abs{\mathcal{S}_t}/N}$ number of disjointed sets $\{\mathcal{S}_{1,t},\mathcal{S}_{2,t}, \ldots, \mathcal{S}_{{\ceil{\abs{\mathcal{S}_t}/N}},t}\}$ such that $\abs{\mathcal{S}_{i,t}} \le N$.}
		\STATE {Divide $\mathcal{S}_t$ to subsets $\{\mathcal{S}_{1,t},\mathcal{S}_{2,t}, \ldots, \mathcal{S}_{{\ceil{\abs{\mathcal{S}_t}/N}},t}\}$ such that $\abs{\mathcal{S}_{i,t}} \le N$ and $\cup_i\mathcal{S}_{i,t}=\mathcal{S}_t$.} \label{proc:ie:divide}
        \FORALL{$\mathcal{S}_{i,t}$}
        \STATE {Individually assign $N$ plays to arms in $\mathcal{S}_{i,t}$ and observe their rewards $R_{k,t}$ for all $k\in\mathcal{S}_{i,t}$.} \label{proc:ie:ie}
        % \Comment{ Exploration}
        \STATE {$\hat{\mu}_{k,t}{\gets} \left(\hat{\mu}_{k,t}(\tau_t-1){+}R_{k,t}\right)/\tau_t$ for all $k$ in $\mathcal{S}_{i,t}.$}
        \ENDFOR
        \STATE{
            $\tau_t \gets \tau_t + 1$, $t\gets t+\ceil{\abs{\mathcal{S}_t}/N}.$
        }
        \ENDPROCEDURE

        \PROCEDURE{United Exploration}{$\mathcal{S}_t', \hat{\bm{\nu}}_t, \iota_t, t$} \label{proc:ue}
        \FORALL{$k\in\mathcal{S}_t'$}
        \STATE {Assign $N$ plays to arm $k$, observe reward $R_{k,t}$.\label{proc:ue:ue}} 
        % \STATE{}
        \STATE $\hat{\nu}_{k,t}\gets \left(\hat{\nu}_{k,t}(\iota_t-1) + R_{k,t}\right)/\iota_t.$
        % \STATE{Update $\hat{{m}}_{k,t}^l$ and $\hat{{m}}_{k,t}^u$ by Eq.(\ref{eq:m_lower_bound}) and Eq.(\ref{eq:m_upper_bound}).}
        \ENDFOR
        \STATE{$\iota_t \gets \iota_t + 1, t\gets t+\abs{\mathcal{S}_t'}.$}
        \ENDPROCEDURE

        \PROCEDURE{Exploitation}{$\mathcal{S}_t,\hat{\bm{m}}_t^l,\hat{\bm{\mu}}_t,\!\hat{L}_t,\!\sigma_t(\!\cdot\!),\tau_t, t$}\label{proc:exploitation}
        % \STATE {\bfseries Input:} Candidate arm set $\mathcal{S}_t$, empirical mean $\hat{\bm{\mu}}$, order mapping $\sigma$, estimated shareable capacities $\hat{\bm{m}}$, and $\hat{L}_t$
        % \STATE Assign plays according to the optimal action $\hat{\bm{a}}_t^*$ derived from $\hat{\bm{m}}_t^l,\hat{\bm{\mu}}_t,\hat{L}_t,\sigma_t(\cdot)$ by Eq.(\ref{eq:optimal_action}).
        \STATE {Assign \(\hat{m}_{\sigma_t(k), t}^l\) plays to arm \(\sigma_t(k)\) for \(k<\hat{L}_t\) and \(N-\sum_{k=1}^{\hat{L}_t-1}\hat{m}_{\sigma_t(k),t}^l\) plays to arm \(\sigma_t(\hat{L}_t)\).}
        % \STATE Assign $\hat{m}_{\sigma(k),t}$ plays to arm $\sigma(k)$ for each $k < \hat{L}_t$ and the remaining $N-\sum_{k=1}^{\hat{L}_t-1}\hat{m}_{\sigma(k),t}^l$ plays to arm $\sigma(\hat{L}_t)$.
        \STATE Observe rewards $R_{\sigma_t(k), t}$ for all $k \le \hat{L}_t.$
        \STATE {$\hat{\mu}_{\sigma_t(k),t}$\\
        ${\gets}\!(\hat{\mu}_{\sigma_t(k),t}(\tau_t{-}1) {+} {R_{\sigma_t(k),t}}/{\hat{m}_{\sigma_t(k), t}^l})/\tau_t\,\text{for}\,k {<} \hat{L}_t$.} 
        \STATE {$\hat{\mu}_{\sigma_t(\hat{L}_t),t} \gets (\hat{\mu}_{\sigma_t(\hat{L}_t),t}(\tau_t-1) $ \\
        $\qquad \quad \quad + {R_{\sigma_t(\hat{L}_t),t}}/{(N-\sum_{k=1}^{\hat{L}_t-1}\hat{m}_{\sigma_t(k),t}^l)})/\tau_t$.}
        % \STATE $\displaystyle \hat{\mu}_{\sigma(\hat{L}_t),t}\gets \left(\hat{\mu}_{\sigma(\hat{L}_t),t}(\tau_t-1) + \frac{R_{\sigma(\hat{L}_t),t}}{N-\sum_{k=1}^{\hat{L}_t-1}\hat{m}_{\sigma(k),t}^l}\right)\big/\tau_t.$
        \STATE{
            $\tau_t \gets \tau_t + 1, t\gets t+1.$
        }
        \ENDPROCEDURE\label{alg:end_proc}
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}[htb]
% 	\caption{Multiple-play successive elimination with shareable arms (\texttt{MP-SE-SA})}
% 	\label{alg:main}
% 	{\bfseries Input:} $K$, $N$, $T$ and two tunable parameters $\gamma \in [1, \infty)$ $\xi \in (0, \infty).$\\
% 	{\bfseries Initial:}
% 	\(t,\tau_t,\iota_t, \gets 1,\, \mathcal{S}_t \gets [K],\, \hat{\bm{\mu}}_t,\hat{\bm{\nu}}_t \gets\bm{0}, \hat{\bm{m}}_t^l \gets \bm{1}, \hat{\bm{m}}_t^l,\hat{\bm{m}}_t^u \gets N\bm{1} ,\,
% 	\hat{L}_t.\)
% 	\begin{algorithmic}[1]
% 		% \STATE {\bfseries Input:} Arm set $[K]$, Multiple-Play $N$, time horizon $T$, and parameters $\gamma\in (1,\infty)$ and $\xi\in (0,1).$   	
% 		\WHILE{$t\le T$}
% 		\IF{$\abs{\mathcal{S}_t}\le N$}
% 		\FORALL{arm $k$ in $\mathcal{S}_t$}
% 		\IF{$\hat{m}_{k,t}^l \neq \hat{m}_{k,t}^u$}
% 		\STATE{Unitedly explore arm $k$ and update $\hat{{\nu}}_{k,t}$. \Comment{Proc.~\ref{alg:ue}}}
% 		\STATE {
% 			$t\gets t+1.$
% 		}
% 		\ENDIF
% 		\ENDFOR
% 		\STATE{Update $\hat{\bm{m}}_{t}^l$ and $\hat{\bm{m}}_{t}^u$ by Eq.(\ref{eq:m_lower_bound}) and Eq.(\ref{eq:m_upper_bound}).}
% 		\STATE{$\iota_t \gets \iota_t + 1.$}
% 		\ENDIF
% 		\STATE{Sort $\{\hat{\mu}_{k,t}, k \in \mathcal{S}_t\}$ via a descending ordering $\sigma$, such that $\hat{\mu}_{\sigma(k),t}$ is the $k$th largest.}
% 		\STATE{Update the expected candidate set size $\hat{L}_t$ by Eq.(\ref{eq:update_L_with_lower_bound}). \label{line:update_L}}
% 		\IF{$\hat{L}_t< \abs{\mathcal{S}_t}$}\label{line:phase_1_2}
% 		\For {$k\in \mathcal{S}_t$ }
% 		\IF {$\hat{\mu}_{k,t} \le \hat{\mu}_{\sigma(\hat{L}_t),t} - \gamma U(\tau_t, T)$}
% 		\STATE $\mathcal{S}_t\gets \mathcal{S}_t\setminus\{k\}.$ \Comment{Elimination}\label{line:elimination}
% 		\ENDIF
% 		\ENDFOR
% 		% \STATE{Update parameter $C$ via Eq.(\ref{eq:update_C}).}
% 		\STATE{Individually explore $\mathcal{S}_t$ and update $\hat{\bm{\mu}}_t.$ \Comment{Proc.~\ref{alg:ie}}}
% 		\STATE{
% 			$\tau_t \gets \tau_t + 1$, $t\gets t+\ceil{\abs{\mathcal{S}_t}/N}.$
% 		}

% 		\ELSIF{$\hat{L}_t= \abs{\mathcal{S}_t}$}\label{line:phase_1_5}
% 		\STATE{Exploit $\mathcal{S}_t$ and update $\hat{\bm{\mu}}_t$. \Comment{Proc.~\ref{alg:exploitation}}}
% 		% \STATE {Assign $N$ plays to arms in $\mathcal{S}_t$ according to their capacities $\hat{\bm{m}}$ and reward mean $\hat{\bm{\mu}}$'s order $\sigma$ \Comment{\scshape Exploitation}}
% 		\STATE{
% 			$\tau_t \gets \tau_t + 1, t\gets t+1.$
% 		}
% 		\ENDIF
% 		% \STATE $\tau\gets \tau + 1$
% 		\ENDWHILE
% 	\end{algorithmic}
% \end{algorithm}

% \begin{procedure}[htb]
% 	\caption{Individual Exploration (IE)}
% 	\label{alg:ie}
% 	\begin{algorithmic}
% 		% \STATE {\bfseries Input:} Candidate arm set $\mathcal{S}_t$, empirical mean $\hat{\bm{\mu}}$  
% 		\STATE{Divide $\mathcal{S}_t$ to $\ceil{\abs{\mathcal{S}_t}/N}$ number of disjointed sets $\{\mathcal{S}_t_1,\mathcal{S}_t_2, \ldots, \mathcal{S}_t_{\ceil{\abs{\mathcal{S}_t}/N}}\}$ such that each $\abs{\mathcal{S}_{i,t}} \le N$.}
% 		\FORALL{$\mathcal{S}_{i,t}$}
% 		\STATE Individually assign $N$ plays to arms in $\mathcal{S}_{i,t}$ and observe their rewards $R_{k,t}$ for all $k\in\mathcal{S}_{i,t}$.
% 		% \Comment{ Exploration}
% 		\STATE $\hat{\mu}_{k,t}\gets \left(\hat{\mu}_{k,t}(\tau_t-1) + R_{k,t}\right)/\tau_t$ for all $k$ in $\mathcal{S}_{i,t}.$
% 		\ENDFOR
% 	\end{algorithmic}
% \end{procedure}

% \begin{procedure}[htb]
% 	\caption{United Exploration (UE)}
% 	\label{alg:ue}
% 	\begin{algorithmic}
% 		\STATE{Update $\hat{m}_{k,t}^u$ via Eq.(\ref{eq:m_upper_bound}).}
% 		\STATE{Assign $\hat{m}_{k,t}^u$ plays to arm $k$ and the rest plays to other top arms in $\mathcal{S}_t$, and observe reward $R_{k,t}$.}
% 		\STATE $\hat{\nu}_{k,t}\gets \left(\hat{\nu}_{k,t}(\iota_t-1) + R_{k,t}\right)/\iota_t$
% 	\end{algorithmic}
% \end{procedure}

% \begin{procedure}[htb]
% 	\caption{Fine-grained Expected Set Size Update}
% 	\label{alg:update_L}
% 	\begin{algorithmic}[1]
% 		\IF{$\xi W(\tau_t, \iota_t, 1/T) \ge 1/2$}\label{line:phase_1_1} \label{line:m_width_start}
% 		\STATE{
% 			Calculate $\hat{m}_{k,t}^l$ via Eq.(\ref{eq:m_lower_bound})
% 			% $\hat{{m}}_{k,t}^{l} \gets \floor{\hat{\nu}_{k,t}/\hat{\mu}_{k,t} - \xi W(\tau_t, \iota_t, 1/T)}\vee 1$ 
% 			for all $k$ in $\mathcal{S}_t.$}
% 		\STATE{
% 			Update $\hat{L}_t$ via Eq.(\ref{eq:update_L_with_lower_bound}).
% 			% $\hat{L}_t \gets \argmin_n\left\{n:\sum_{k=1}^n \hat{m}_{\sigma(k)}^{l}\ge N\right\}.$
% 		}
% 		\ELSIF{$\xi W(\tau_t, \iota_t, 1/T) < 1/2$}\label{line:phase_2}
% 		\STATE{
% 			Calculate $\hat{m}_{k,t}$ via Eq.(\ref{eq:rounding_estimator}) for all $k$ in $\mathcal{S}_t$.
% 			% $\hat{{m}}_{k,t} \gets \round{\hat{\nu}_{k,t} / \hat{\mu}_{k,t}}$ for all $k$ in $\mathcal{S}_t.$
% 		}
% 		\STATE{
% 			Update $\hat{L}_t$ via Eq.(\ref{eq:update_L_at_last}).
% 			% $\hat{L}_t\gets \argmin_n\left\{n:\sum_{k=1}^n \hat{m}_{\sigma(k),t}\ge N\right\}.$
% 		}
% 		\ENDIF \label{line:m_width_end}
% 	\end{algorithmic}
% \end{procedure}


% \begin{procedure}[htb]
% 	\caption{Individual Exploration (IE)}
% 	\label{alg:ie}
% 	\begin{algorithmic}
% 		% \STATE {\bfseries Input:} Candidate arm set $\mathcal{S}_t$, empirical mean $\hat{\bm{\mu}}$  
% 		\STATE{
% 		Divide $\mathcal{S}_t$ to $\ceil{\abs{\mathcal{S}_t}/N}$ number of disjointed sets $\{\mathcal{S}_t_1,\mathcal{S}_t_2, \ldots, \mathcal{S}_t_{\ceil{\abs{\mathcal{S}_t}/N}}\}$ such that each $\abs{\mathcal{S}_{i,t}} \le N$.}
% 		\ForALL{$\mathcal{S}_{i,t}$}
% 		\STATE Individually assign $N$ plays to arms in $\mathcal{S}_{i,t}$ and observe their rewards $R_{k,t}$ for all $k\in\mathcal{S}_{i,t}$.
% 		% \Comment{\scshape Exploration}
% 		\STATE $\hat{\mu}_{k,t}\gets (\hat{\mu}_{k,t}(\tau-1) + R_{k,t})/\tau$ for all $k$ in $\mathcal{S}_{i,t}.$
% 		\ENDFOR
% 	\end{algorithmic}
% \end{procedure}

% \begin{procedure}[htb]
% 	\caption{United Exploration (UE)}
% 	\label{alg:ue}
% 	\begin{algorithmic}
% 		% \STATE {\bfseries Input:} Candidate arm set $\mathcal{S}_t$, empirical mean $\hat{\bm{M}}$   
% 		\For{$k\in \mathcal{S}_t$}
% 		\STATE{
% 			Update $\hat{m}_{k,t}^u$ via Eq.(\ref{eq:m_upper_bound}).
% 			% $\hat{m}_{k,t}^{u} \gets \ceil{\hat{\nu}_{k,t}/\hat{\mu}_{k,t} + \xi W(\tau_t, \iota_t, 1/T)}\wedge N$.
% 		}
% 		\STATE{	Assign $\hat{m}_{k,t}^u$ plays to arm $k$ and the rest plays to other top arms in $\mathcal{S}_t$, and observe reward $R_{k,t}$ from arm $k$.}
% 		\STATE{
% 			Update $M$ via Eq.(\ref{eq:update_M}).
% 			% $M\gets \max\{\hat{m}_{k,t}^{u}, k\in \mathcal{S}_t\}$.
% 		}
% 		\ENDFOR
% 	\end{algorithmic}
% \end{procedure}

% \begin{procedure}[htb]
% 	\caption{Exploitation}
% 	\label{alg:exploitation}
% 	\begin{algorithmic}
% 		% \STATE {\bfseries Input:} Candidate arm set $\mathcal{S}_t$, empirical mean $\hat{\bm{\mu}}$, order mapping $\sigma$, estimated shareable capacities $\hat{\bm{m}}$, and $\hat{L}$
% 		\STATE Assign $\hat{m}_{\sigma(k)}$ plays to arm $\sigma(k)$ for each $k < \hat{L}$ and the rest $N-\sum_{k=1}^{\hat{L}-1}\hat{m}_{\sigma(k)}$ plays to arm $\sigma(\hat{L})$.
% 		\STATE Observe rewards $R_{\sigma(k), t}$ for all $k \in \{1,2,\ldots, \hat{L}\}.$
% 		\STATE $\hat{\mu}_{\sigma(k)}\gets (\hat{\mu}_{\sigma(k)}(\tau-1) + R_{\sigma(k),t}/\hat{m}_{\sigma(k)})/\tau$ for $k < \hat{L}.$
% 		\STATE $\hat{\mu}_{\sigma(\hat{L})}\gets (\hat{\mu}_{\sigma(\hat{L})}(\tau-1) + R_{\sigma(\hat{L}),t}/(N-\sum_{k=1}^{\hat{L}-1}))/\tau.$
% 	\end{algorithmic}
% \end{procedure}

% \textbf{Two tuneable parameters.} To enhance the algorithm's efficiency, we add two parameters: $\gamma \ge  1$ for scaling $\gamma U(\tau_t, T)$ and $\xi > 0$ for scaling UCI's failure probability as $2\xi/T$.
% The smaller the $\gamma$ the more aggressive in eliminating arms, while the smaller the $\xi$ the more conservative in estimating capacities.
% $\gamma$ and $\xi$ can be tuned for better performance in a specIfic environment but simply setting both as $1$ is also valid.
% Their impact on regret bounds is shown in Section~\ref{sec:analysis}.
%  $W(\tau_t, \iota_t, 1/T; M, C)$.

% \textbf{Update $M$ and $C$ for UCI width.}
% % Notice that as we apply $W(\tau_t, \iota_t, 1/T)$ is a unIForm confidence interval's width. 
% Initially, we set $M=N$ and set $C$ as a small positive value.
% During the learning process, inferior arms will be eliminated, so we can update $M$ and $C$ for arms in the candidate set $\mathcal{S}_t$.
% As the width $W(\tau_t, \iota_t, 1/T)$ decreases, we calculate the upper bound of service capacities as follows,
% \begin{equation}\label{eq:m_upper_bound}
% 	\hat{m}_{k,t}^{u}=\min \{\ceil{\hat{\nu}_{k,t}/\hat{\mu}_{k,t} + W(\tau_t, \iota_t, 1/T)}, N\},
% \end{equation}
% and update $M$ to
% \begin{equation}\label{eq:update_M}
% 	M
% 	=
% 	\max\{\hat{m}_{k,t}^{u}, k\in \mathcal{S}_t\}.
% \end{equation}
% Similarly, as set $\mathcal{S}_t$ reduces, we can update $C$ as the highest reward mean estimates of those eliminated arms, that is
% \begin{equation}\label{eq:update_C}
% 	C=\max\left\{\hat{\mu}_{k,t}, k\in [K]\setminus \mathcal{S}_t\right\}.
% \end{equation}
% Such update guarantees $M$ is the upper bound of capacities and $C$ is a lower bound of reward means for arms in $\mathcal{S}_t$, i.e., $M \ge m_k, C \le \mu_k$ for all arm $k\in\mathcal{S}_t$, with high probability.
% The UCI's width in Eq.(\ref{eq:m_interval_width}) is increasing (decreasing) with respect to $M$ ($C$), and $M$ ($C$) decreases (increases) as time elapses.
% So, this update further reduces UCI's width.



% \textbf{Two tuneable parameters} The algorithm contains two tuneable parameters $\gamma\ge 1$ for arm elimination gap $U(\tau_t, T)$ and $0<\xi\le 1$ for estimated sharing capacities' confidence width $W(\tau_t, \iota_t, 1/T)$, in which $\gamma = 1$ is the most aggressive in eliminating arms and $\xi=1$ is the most conservative in estimating capacities. In Section~\ref{sec:analysis}, we illustrate their impact in regret upper bound $W(\tau_t, \iota_t, 1/T; M, C)$.



% for decoupling both learning tasks, let's first consider how explore-then-commit (ETC) algorithm in MAB decouple the exploration and exploitation trade-off. That is, set a stopping time, beFore the time slot, do exploration either unIFormly or according to some rules, and then after the stopping time we do exploitation.
% Such policy directly decouple the two aspect of exploration and exploitation trade-off, but turns off to be suboptimal~\citep{garivier_explore-then-commit_2016}.
% Then, when it turns to UCB or Thompson sampling, with well designed index expression, both can achieve optimal perFormance.

% This observation provides the insight that policies that clearly decouple or separate two tasks in sequential decision making, though provides an easy design to solve the problem, is worse than indexes policies which implicitly inherit both coupled tasks, exploitation and exploration in MAB, and learning reward mean and sharing capacity in our MP-MAB-SE model.

% So basically, though we do want to decouple our two learning tasks, we have to be careful when doing that for the clearer a decouple is, the costlier a policy is (the higher the regret is).

% Another alternative 
% A absolutely decoupled design would be applying Section~\ref{sec:learning_sharing_capacity}'s estimator first to obtain good estimates of sharing capacity as the first phase, then in the second phase turn to learning reward mean.
% That is, based on Corollary~\ref{cor:m_sample_complexity}'s estimator sample complexity result,
% one first spends $K(1/N+\ceil{{K}/{N}}) \times O((N^2/C^2)\log T)$ time slots\footnote{
% 	Notice that upper bound of sharing capacity $M$ is unknown, so we have to use $N$ as the upper bound in the sample complexity in ETC.
% }
% to per palely and unitedly explore each arm and estimate their sharing capacities $\hat{m}_{k,t}$ accurately,
% and then adapt a MP-MAB algorithm (e.g. CUCB or MP-TS)
% to the shareable arm setting to further update per play reward mean estimates.
% We call such design as ETC since this design follows the same decouple idea of ETC;s in MAB.
% Such design would immediately causes a $\O((K^2N{\color{red}+KNM})\log T)$
% regret\footnote{Draft:
% 	% the latter part should be updated, CUCB is much complex than $1/\Delta^2$.
% 	the proof is done. But still need to check.
% } (see Appendix~\ref{appsub:etc_ucb}).
% However, this exploration strategy is crude and not efficient.

% A slightly better approach would be to consider to concentrate explorations to potential good arms.
% That is, add a pre-processing phase to per palely explore arms' per play reward means
% and then eliminate these signIficant suboptimal arms
% (i.e., with a descending order, arms with $\{N+1, N+2,\ldots, K\}$ indexes).
% Then, turn to explore those candidate arms' sharing capacity and reward means as ETC does.
% Notice that the optimal action only allocate plays to top $L$ arms where $L$ may be much smaller than $N$.
% So, such idea is still kind of coarse and motive us to take a further step.
% In this approach, we start from exploring reward mean, and then sharing capacity, and at least back to reward mean.
% So, this design is better than the ETC one, for it does not separate both tasks so clear.
% We call this algorithm as \texttt{MP-SE-SA} (na\"ive).

% Notice that both ideas requires an almost clear decoupling between \texttt{MP-MAB-SA}'s two learning task, so both of them must cause a higher regret for such coarse-grained designs.



% is the explore-then-commit (ETC) approach~\citep{garivier_explore-then-commit_2016}.
% Based on Corollary~\ref{cor:m_sample_complexity},
% one can first spend $K(1/N+\ceil{{K}/{N}}) \times O((N^2/C^2)\log T)$ time slots\footnote{
% 	Notice that upper bound of sharing capacity $M$ is unknown, so we have to use $N$ as the upper bound in the sample complexity in ETC.
% }
% to individually and unitedly explore each arm and estimate their sharing capacities $\hat{m}_{k,t}$ accurately,
% and then adapt an MP-MAB algorithm (e.g. CUCB or MP-TS)
% to the shareable arm setting to further update individual reward mean estimates.

%In Section~\ref{sec:analysis}, we show that our algorithm enjoys much smaller coefficients.



% \subsection{Design Overview}

% We apply the UCI derived in last section to design algorithms
% to solve \texttt{MP-MAB-SA}.
% The key challenge is to balance the exploration vs. exploitation tradeoff.


% A slightly better approach would be to consider to concentrate explorations to potential good arms.
% That is, add a pre-processing phase to individually explore arms' per play reward means
% and then eliminate these signIficant suboptimal arms
% (i.e., with a descending order, arms with $\{N+1, N+2,\ldots, K\}$ indexes).
% Then, turn to explore those candidate arms' sharing capacity and reward means as ETC does.
% Notice that the optimal action only allocate plays to top $L$ arms where $L$ may be much smaller than $N$.
% So, such idea is still kind of coarse and motive us to take a further step.

% To improve the exploration efficiency,
% we apply the successive elimination (SE) approach
% developed for classical MAB \citep{perchet_multi-armed_2013}
% to design our \texttt{MP-SE-SA} algorithm.
% In the design of \texttt{MP-SE-SA},
% we address the following challenges.
% First, instead of knowing the number of arms to eliminate as the classical MAB setting,
% % our MAB setting with sharable arms and multiple plays,
% in \texttt{MP-MAB-SA},
% the number of arms to be eliminated is unknown in advance.
% IF eliminating too much arms, left arms will be insufficient, leading to a linear regret.
% IF eliminate too less arms, we have to explore suboptimal arms often which also leads to additional costs.
% Furthermore, the number of arms to be eliminated is determined by the sharing capacity
% and the individual mean, both of which are unknown.
% Also, multiple plays in each round makes the exploration more complicated.
% One needs to decide the number of plays for each arm,
% which influences the estimation of sharing capacity and individual reward mean.
% We present our \texttt{MP-SE-SA} algorithm in Algorithm~\ref{alg:main} and its three subroutines: united exploration (UE) in PROCEDURE~\ref{alg:ue}, individual exploration (IE) in PROCEDURE~\ref{alg:ie}, and exploitation in PROCEDURE~\ref{alg:exploitation}\footnote{Draft: or we can move these procedures to Appendix, as they are too trivial to occupy space.}.



% \subsection{The \texttt{MP-SE-SA} Algorithm}

% \subsection{Our Algorithm}	
%Recall that $L$ is the smallest number of top arms 
%whose capacities together can cover all $N$ plays (see Eq.(\ref{eq:critical_top_arms})), 
%$L$ is less than the number of plays $N$ 
%and the number number of plays $N$ is less than the total number of arms $K$ (i.e., $L< N < K$).   
%Since the arm ordering $\mu_1 > \mu_2 > \ldots > \mu_K$ is also assumed, the top arm set is $[L]\coloneqq\{1,2,\ldots, L\}$ and the rest arms (with indexes greater than $L$) are \textit{suboptimal}.



%\textbf{Algorithm overview.} 

% We specIfy UCI's width $W(\tau_{k,t}, \iota_{k,t}, \delta)$ derived in Lemma~\ref{lma:ufc_m} as $\xi W(\tau_{k,t}, \iota_{k,t}, 1/T)$, where $0<\xi\le 1$ is a control parameter for our sharing capacity estimator's aggressiveness, and we also set $\delta=1/T$ for an adaptive interval width.


% Recall from Section \ref{sec:model} that $L$ is the smallest number of top arms
% whose capacities together can cover all $N$ plays (see Eq.(\ref{eq:critical_top_arms})),
% the optimal arm set is $[L]\coloneqq\{1,2,\ldots, L\}$
% and the rest arms (with indexes greater than $L$) are \textit{suboptimal}.
% Our algorithm's main idea is as follows.
% It is initialized with a candidate arm set $\mathcal{S}_t = [K]$.
% In each phase (contains of $|\mathcal{S}_t|$ time slots),
% explore (IE or UE determined by the algorithm) each arm in $\mathcal{S}_t$ once
% and then use the feedback (or reward) to update estimations of individual reward mean and sharing capacity.
% Between these exploration phases, successively eliminate suboptimal arms from $\mathcal{S}_t$
% according to \textit{two conditions} until the candidate set $\mathcal{S}_t=[L]$.
% % only containing the top-$L$ arms (i.e. $\mathcal{S}_t$ equal to $[L]$).
% % maintain a candidate arm set $\mathcal{S}_t$ initialized as the whole arm set $[K]$, and  
% % The algorithm's aim is to reduce candidate arm set's size $\abs{\mathcal{S}_t}$ to $L$ both effectively and safely (i.e., with high correct probability). 
% The first conditions is to make assure that the sharing capacities $m_k$
% of arms in the candidate set $\mathcal{S}_t$ can cover all $N$ plays.
% This depends on our sharing capacity's estimation $\hat{m}_{k,t}$ and the confidence interval width $W(\tau_{k,t}, \iota_{k,t}, 1/T)$.
% The second condition requires one to eliminate suboptimal arms with high accuracy.
% This relies upon our elimination criterion and empirical individual reward mean $\hat{\mu}_{k,t}$.
% % these suboptimal arm's empirical reward mean should be clearly smaller then these top arms so to eliminate them.
% Since all arms $k$ in the candidate set $\mathcal{S}_t$ have the same number of IE $\tau_{k,t}$ and UE $\iota_{k,t}$,
% we omit the subscript $k$ and simplIfy them as $\tau_t$ and $\iota_t$
% and update them recursively.



% we should shirk the expected candidate arm set size $\hat{L}$ to $L$ in the learning procedure (see Figure~\ref{fig:size_update}).  



% \textbf{Update expected candidate set size.}
% A key element of our algorithm design is to effectively reduce the expected candidate set size.
% We denote $\hat{L}_t$ as the expected size of candidate set $\mathcal{S}_t$ with observations up to time slot $t$.
% It means with current statistics, one assures that the sharing capacities of these top $\hat{L}_t$ arms in the candidate set can covers all $N$ plays. We can achieve the first condition as long as the candidate set's size $\abs{\mathcal{S}_t}$ is no less than the expected size $\hat{L}_t$.

% Figure~\ref{fig:size_update} depicts the expected size $\hat{L}_t$'s update in \texttt{MP-SE-SA} (red line) and compare it with ETC (green line) and MP-SE (blue line). The details of ETC and MP-SE are deferred to Appendix~\ref{app:simple_algo}.
% The improvement of \texttt{MP-SE-SA} upon MP-SE is attributed to the unIForm confidence interval. With a unIFormly applicable interval in the learning process, we can reduce the expected candidate arm set size during exploration with a high correctness probability.
% The improvement of MP-SE comparing to ETC is from successive elimination: during exploration,
% we eliminate obviously suboptimal arms with small empirical reward means, and thus saves the cost of exploration.
% % We omit the variable $t$ of $\hat{L}_t$ when no confusion is possible.

% \begin{figure}[htb]
% 	\centering
% 	\includegraphics[width=0.47\textwidth]{figures/L_comparision.pdf}
% 	\caption{The update of expected size $\hat{L}$ for candidate set $\mathcal{S}_t$}
% 	\label{fig:size_update}
% \end{figure}

% % As mentioned beFore, we should make sure the top $\hat{L}$ arms' sharing capacities can cover all $N$ plays.
% At the start of our algorithm, without any inFormation, we simply set $\hat{L}=N$ to make sure the candidate arms can cover all $N$ plays.
% % expect to keep $N$ arms in candidate set $\mathcal{S}_t$, i.e., $\hat{L}=N$, so to cover all $N$ plays. 
% % As our learning proceeds, 
% % we would be able to have estimation of sharing capacity $\hat{m}_{k,t}$.  
% % As our unIForm confidence interval holds for all time slots,
% As the algorithm proceeds and the unIForm confidence interval becomes narrow,
% we calculate the lower bound for the estimator of sharing capacity as
% \begin{equation}\label{eq:m_lower_bound}
% 	\hat{m}_{k,t}^{{l}}=\floor{\hat{\nu}_{\sigma(k), t}/\hat{\mu}_{\sigma(k), t} - W(\tau_t, \iota_t, 1/T)}\vee 1,
% \end{equation}
% for arms $k$ in set $\mathcal{S}_t$ and use them to improve the expected size $\hat{L}$.
% Denote empirical individual reward means' order descending map as $\sigma_t(\cdot)$.
% The expected size would be
% \begin{equation}\label{eq:update_L_with_lower_bound}
% 	\hat{L}_t=\argmin_n\left\{n, \sum_{k=1}^n \hat{m}_{\sigma(k),t}^{{l}} \ge N\right\}.
% \end{equation}
% Later on, when $W(\tau_t, \iota_t, 1/T) < 1/2$, the estimations of sharing capacities as $\hat{m}_{k,t}$
% becomes accurate enough. We then obtain the smallest expected size
% \begin{equation}\label{eq:update_L_at_last}
% 	\hat{L}_t= \argmin_n\left\{n, \sum_{k=1}^n \hat{m}_{\sigma(k),t} \ge N\right\},
% \end{equation}
% and with high probability, $\hat{L}_t= L$.

% \textbf{The elimination criterion} We apply the elimination criterion by~\citep{perchet_multi-armed_2013}. It corresponds to the second condition. for any arm $k$ in candidate set $\mathcal{S}_t$, IF its empirical individual reward mean $\hat{\mu}_{k,t}$ is much worse than the $\hat{L}_t$-th largest empirical reward mean, that is
% %  fulfill the following inequality
% \begin{equation*}
% 	\hat{\mu}_{k,t} \le \hat{\mu}_{\sigma(\hat{L}),t} - \gamma U(\tau_t, T),
% \end{equation*}
% we eliminate the arm $k$ from the candidate set $\mathcal{S}_t$. The function $U(\tau_t, T)$ is a high confidence upper bound on the deviation of $\hat{\mu}_{k,t} - \hat{\mu}_{\sigma(\hat{L})}$ from $\mu_k - \mu_{\sigma(\hat{L}),t}$ and $\tau$ is the IE times for the candidate set. Its detail Formula is
% \begin{equation}\label{equ:mu_interval_width}
% 	U(\tau_t, T) \coloneqq 2\sqrt{\frac{2}{\tau_t}\xoverline{\log} \left(\frac{T}{\tau_t}\right)},
% \end{equation}
% where $\xoverline{\log}(x) = \max\{\log x, 1\}$.
% % for any two arm $k  > l$ both with $\tau$ times of IE, that's a high confidence upper bound on the deviation of $\hat{\mu}_{k,t} - \hat{\mu}_l$ from $\mu_k - \mu_l$.
% %  and $a\vee b = \max\{a,b\}$.	
% % make sure the confidence interval width is less than half to guarantee the correct estimation. 

% See Figure~\ref{fig:size_update}. It show how our algorithm (\texttt{MP-SE-SA}) be able to reduce the arm set size $\hat{L}$ much faster than other algorithms, i.e. ETC and basic MP-SE algorithm (see Appendix~\ref{app:simple_algo}). 

% The elimination consists of two phases. 
% \textit{\underline{Phase 1}:} 
% eliminate suboptimal arms $k$ in $\{N+1, N+2, \ldots, K\}$. 
% \textit{\underline{Phase 2}:}  when the estimations of sharing capacities $\hat{m}_{k,t}$ are accurate, estimate $\hat{L}$ and eliminate the rest suboptimal arms $k$ in $\{\hat{L}+1, \hat{L}+2, \ldots, N\}$.
% Note that there may exist an {intermediate} phase (\underline{\textit{Phase 1.5}}) between the above two elimination phases, that is, when the candidate arm set $\mathcal{S}_t$ contains $N$ arms (i.e., phase 1 ends) but the estimations $\hat{m}_{k,t}$ are inaccurate (i.e., phase 2 doesn't start). In phase 1.5, the algorithm would keep applying IE and UE for arms in candidate set $\mathcal{S}_t$ to accumulate observations. 
% % Note that when the algorithm processing, there may not exist a clear separation of both phases. for example, the algorithm may be able to estimate $\hat{m}_{k,t}$ with high confidence when the candidate arm set's size $\abs{\mathcal{S}_t}$ is still greater than $N$.   


% The elimination consists of two main phases. 
% \underline{\textit{Phase 1:}} the algorithm would first assume the sharing capacities 
% % when the algorithm isn't able to estimate arms' sharing capacities $m_k$ with confidence, it would assume 
% $\hat{m}_{k,t} = 1$, use IE and UE to learn $\hat{m}_{k,t}$ and the individual reward mean $\hat{\mu}_{k,t}$, and eliminate suboptimal arms $k$ in $\{N+1, N+2, \ldots, K\}$ according to $\hat{\mu}_{k,t}$. 
% \underline{\textit{Phase 2:}} when the estimation of capacities $\hat{m}_{k,t}$ are accurate enough, the algorithm eliminates the rest suboptimal arms $k$ in $\{L+1, L+2, \ldots, N\}$ and stop UE. 
% Note that there may exist an {intermediate} phase (\underline{\textit{Phase 1.5}}) between the above two, that is, when the candidate arm set $S$ only contains $N$ arms (i.e., phase 1 ends) but the estimations $\hat{m}_{k,t}$ are still inaccurate (i.e., phase 2 doesn't start). In phase 1.5, the algorithm would keep applying IE and UE to accumulate observations. 
% % Note that when the algorithm processing, there may not exist a clear separation of both phases. for example, the algorithm may be able to estimate $\hat{m}_{k,t}$ with high confidence when the candidate arm set's size $\abs{\mathcal{S}_t}$ is still greater than $N$.   

% To estimate sharing capacities $m_k$, we apply the criterion derived in Lemma~\ref{lma:learning_m_criterion}. That is, apply the rounding estimator in Eq.(\ref{eq:rounding_estimator}) when the IE and UE sample sizes $\tau$ and $\iota$ can assure $W(\tau,\iota, T) < 1/2$.



% One can regards the algorithm has two modes, it depends on whether we have get the reliable estimation of sharing capacities $m_k$. When $\xi W(\tau_t, \iota_t, 1/T) \ge 1/2$, we eliminate arms $\{N+1, N+2, \ldots, N\}$. Recall that we are arm to eliminate all other arms except top $L$ arms.
% When $\xi W(\tau_t, \iota_t, 1/T) < 1/2$, we further eliminate arms $\{L+1, L+2, \ldots, N\}$. 

% The mode depends on Line~\ref{line:mode_start}-\ref{line:mode_end}.

% In each mode, IF the current number of arms in the candidate arm set $\mathcal{S}_t$ is larger than $\hat{L}$ the number we expected, we would check whether it can be eliminated in Line~\ref{line:elimination}.


% \subsection{Relax Assumptions}

% give a complexer exploration to replace the old one in order to relax the first assumption;

% show how to relax the second assumption and not hurt the algorithm;

% \subsection{Improved Algorithms}

% There are two further improvement of the Algorithm~\ref{alg:main}; both update are possible for we use the unIForm confidence interval technique in sharing capacity estimation part. 

% First, replace Algorithm~\ref{alg:main}'s Line~\ref{line:simple_m_estimate} with the following:
% \begin{algorithmic}
% 	\STATE{
% 		$\hat{{m}}_{k,t} \gets \floor{\hat{\nu}_{k,t}/\hat{\mu}_{k,t} - \xi W(\tau_t, \iota_t, 1/T)}\vee 1$ for all $k$ in $\mathcal{S}_t.$
% 	}
% \end{algorithmic}

% Second, replace the UE PROCEDURE~\ref{alg:ue}'s Line~\ref{line:ue_tobe_update} with the following:
% \begin{algorithmic}
% 	\STATE{$\hat{m}_{k,t}^{u} \gets \ceil{\hat{\nu}_{k,t}/\hat{\mu}_{k,t} + \xi W(\tau_t, \iota_t, 1/T)}\wedge N$.}
% 	\STATE{
% 		Assign $\hat{m}_{k,t}^u$ plays to arm $k$ and the rest plays to other top arms in $\mathcal{S}_t$, and observe reward $R_{k,t}$ from arm $k$.
% 	}
% \end{algorithmic}

% Answered: I will update the learning sharing capacity part with unIForm confidence bound
% \begin{remark}[Draft]
% 	The algorithm can be further refined in two aspects (i.e. lower bound of $m_k$ for elimination and upper bound of $m_k$ for exploration), we will give it in the \textbf{appendix}. 	
% 	\textbf{Question?} Do we still do that? In our Appendix, we also show a refined algorithm in which the sharing capacity's confidence interval plays a more important part. 
% 	The \textbf{problem} is that such refinement has No logarithmic regret, or we may need to replace Lemma~\ref{lma:learning_m_criterion}'s technique with unIForm confidence intervals (martingales).
% \end{remark}

